PC-MLP: Model-based Reinforcement Learning with Policy Cover Guided Exploration

Model-based Reinforcement Learning (RL) is a popular learning paradigm due to its potential sample efficiency compared to model-free RL. However, existing empirical model-based RL approaches lack the ability to explore. This work studies a computationally and statistically efficient model-based algorithm for both Kernelized Nonlinear Regulators (KNR) and linear Markov Decision Processes (MDPs). For both models, our algorithm guarantees polynomial sample complexity and only uses access to a planning oracle. Experimentally, we first demonstrate the flexibility and efficacy of our algorithm on a set of exploration challenging control tasks where existing empirical model-based RL approaches completely fail. We then show that our approach retains excellent performance even in common dense reward control benchmarks that do not require heavy exploration. Finally, we demonstrate that our method can also perform reward-free exploration efficiently. Our code can be found at https://github.com/yudasong/PCMLP.

==> eluder_app.tex <==
\section{Sample Complexity Analysis with Distribution Eluder Dimension}

%We provide detailed analysis for complexity complexity 

We start with a concentration lemma which shows the feasibility of the ground truth model $P^\star$ throughout the entire learning process.
\begin{lemma}[Feasibility of $P^\star$] \label{lem:feasibility} Fix $\delta \in (0,1)$. With probability at least $1-\delta$, for all $n\in [N]$, we have:
\begin{align*}
P^\star \in \Pcal_{n}.
\end{align*} Also for any $P \in \Pcal_n$, we have:
\begin{align*}
\EE_{s,a\sim d^{\boldpi_n}} \left\| P(\cdot |s,a) - P^\star(\cdot | s,a)  \right\|^2_1 \leq 6 \sqrt{\frac{ \ln(2 |\Pcal| N /\delta)  }{M}} + \frac{ 2\ln\left(2 |\Pcal| N / \delta \right)  }{M}.
\end{align*}
\end{lemma}
\begin{proof}
Denote failure probability for each iteration as $\delta / (2N)$. From the MLE guarantee (Theorem 21 from \cite{agarwal2020flambe}), we have that:
\begin{align*}
\EE_{s,a\sim d^{\boldpi_n}} \left\| \widehat{P}_n(\cdot | s,a) - P^\star(\cdot | s,a) \right\|_1^2 \leq \frac{ 2\ln\left( 2 |\Pcal| N / \delta \right)  }{M},
\end{align*} with probability at least $1-\delta/(2N)$. 

Recall that the confidence ball is build using another i.i.d $M$ samples $(s,a,s')$ from $d^{\boldpi_n}P^\star$. Thus the samples used to construct the confidence ball is independent of $\widehat{P}_n$.  Thus we have that for all $P\in\Pcal$:
\begin{align*}
\left\lvert \frac{1}{M} \sum_{i=1}^M \left\| P(\cdot | s_i,a_i) - \widehat{P}_n(\cdot |s_i,a_i)\right\|^2_{1} - \EE_{s,a\sim d^{\boldpi_n}} \left\| P(\cdot | s,a) - \widehat{P}_n(\cdot | s,a) \right\|_1^2 \right\rvert \leq 4 \sqrt{\frac{ \ln( 2 |\Pcal| N /\delta)  }{M}},
\end{align*} with probability at least $1-\delta / (2N)$. Thus, it means that for $P^\star$:
\begin{align*}
\frac{1}{M} \sum_{i=1}^M \left\| P^\star(\cdot | s_i,a_i) - \widehat{P}_n(\cdot | s_i,a_i) \right\|_1^2 & \leq 4 \sqrt{\frac{2 \ln(|\Pcal| N /\delta)  }{M}} + \EE_{s,a\sim d^{\boldpi_n}} \left\| \widehat{P}_n(\cdot | s,a) - P^\star(\cdot | s,a) \right\|_1^2\\
& \leq 4 \sqrt{\frac{ \ln(2 |\Pcal| N /\delta)  }{M}} + \frac{ 2\ln\left(2 |\Pcal| N / \delta \right)  }{M},
\end{align*}  which matches to the confidence interval we set. 
This implies that $P^\star \in \Pcal_n$ with probability at least $1-\delta/N$.   

On the other hand, this also means that for any $P\in \Pcal_n$, we must have:
\begin{align*}
\EE_{s,a\sim d^{\boldpi_n}} \left\| P(\cdot | s,a) - \widehat{P}_n(\cdot | s,a)  \right\|_1^2 & \leq 4 \sqrt{\frac{ \ln(2 |\Pcal| N /\delta)  }{M}} + \frac{1}{M} \sum_{i=1}^M \left\| P^\star(\cdot | s_i,a_i) - \widehat{P}_n(\cdot | s_i,a_i) \right\|_1^2 \\
& \leq 6 \sqrt{\frac{ \ln(2 |\Pcal| N /\delta)  }{M}} + \frac{ 2\ln\left(2 |\Pcal| N / \delta \right)  }{M}.
\end{align*}


Applying union bound over all $N$ rounds concludes the proof. 
\end{proof}

Let us denote $(\pi_{n+1}, \widetilde{P}_{n+1}) = \argmax_{\pi\in\Pi, P\in\Pcal_n} V^{\pi}_{P}$. The feasibility lemma above (Lemma~\ref{lem:feasibility}) implies that $\pi_{n+1}$ is an optimistic policy in the sense that $V^{\pi_{n+1}}_{\widetilde{P}_{n+1}} \geq V^\star$.

\begin{lemma}Assume the condition in Lemma~\ref{lem:feasibility} holds. Then for all $n\in [N]$, we must have $V^{\pi_{n+1}}_{\widetilde{P}_{n+1}} \geq V^\star$.
\end{lemma}
The proof of the above lemma is simply the combination of $P^\star$ being in $\Pcal_n$ and the $\pi_{n+1}, \widetilde{P}_n$ are the maximizers of the constrained optimization program. 

Now we can use the distributional Eluder dimension to bound the number of total rounds where $\pi_{n+1}$ is not an $\epsilon$-near optimal policy, i.e., $V^{\pi_{n+1}} \leq V^\star - \epsilon$.


\begin{lemma}[Bounding number of sub-optimal rounds] Assume Lemma~\ref{lem:feasibility} holds. Setting number of samples per iteration $M = \frac{256 d_{\epsilon}^2 \ln( 2|\Pcal| d_{\epsilon}/\delta)  }{\epsilon^4} + \frac{8 d_{\epsilon} \ln(2 |\Pcal| d_{\epsilon} /\delta )  }{\epsilon^2}$,  with probability at least $1-\delta$, we have that $N \leq d_{\epsilon}$, and there exists $n\in [N]$, such that $V^{\pi_n} \geq V^\star - \epsilon$.
\end{lemma}
\begin{proof}Consider iteration $n$ where $V^{\pi_{n}} \leq V^\star - \epsilon$.
By optimism, we have:
\begin{align*}
\epsilon \leq V^\star - V^{\pi_{n}} & \leq  V^{\pi_n}_{\widetilde{P}_n} - V^{\pi_n} = \sum_{h=0}^{H-1} \EE_{s,a\sim d^{\pi_n}_h} \left[ \EE_{s'\sim \widetilde{P}_n(\cdot|s,a)} V^{\pi_n}_{\widetilde{P}_n;h+1}(s') -   \EE_{s'\sim {P}^\star(\cdot|s,a)} V^{\pi_n}_{\widetilde{P}_n;h+1}(s')   \right] \\
& \leq  H \EE_{s,a\sim d^{\pi_n}} \left\| \widetilde{P}_n(\cdot | s,a) - P^\star(\cdot | s,a)   \right\|_{1},
\end{align*} which implies that:
\begin{align*}
\EE_{s,a\sim d^{\pi_n} } \left\| \widetilde{P}_n(\cdot | s,a) - P^\star(\cdot | s,a)  \right\|_{1} \geq \frac{\epsilon}{H}.
\end{align*}
Note that $\widetilde{P}_n \in \Pcal_{n-1}$ and $P^\star \in \Pcal_{n-1}$, which means that:
\begin{align*}
&\EE_{s,a\sim d^{\boldpi_{n-1}}} \left\|  \widetilde{P}_n(\cdot | s,a) - P^\star(\cdot | s,a) \right\|^2_{1} \\
&  \leq 2 \EE_{s,a\sim d^{\boldpi_{n-1}}} \left\|  \widetilde{P}_n(\cdot | s,a) - \widehat{P}_{n-1}(\cdot | s,a) \right\|^2_{1}  + 2 \EE_{s,a\sim d^{\boldpi_{n-1}}} \left\|  \widehat{P}_{n-1}(\cdot | s,a) - P^\star(\cdot | s,a) \right\|^2_{1}  \leq 4\delta. 
\end{align*}
Note that $d^{\boldpi_{n-1}} = \sum_{i=0}^{n-1} d^{\pi_i} / n$. This means that:
\begin{align*}
 \sum_{i=0}^{n-1} \EE_{s,a\sim d^{\pi_i}}  \left\| \widetilde{P}_{n}(\cdot|s,a) - P^\star(\cdot | s,a)  \right\|_{1}^2  \leq 4 n \delta.
\end{align*} Using the fact that $(\EE[x])^2 \leq \EE[x^2]$, we have:
\begin{align*}
\sqrt{ \sum_{i=0}^{n-1} \left( \EE_{s,a\sim d^{\pi_i}}  \left\| \widetilde{P}_{n}(\cdot|s,a) - P^\star(\cdot | s,a)  \right\|_{1} \right)^2   } \leq 2\sqrt{ n \delta}.
\end{align*}
Assume that we set $\delta$ properly such that $2\sqrt{n \delta} \leq \epsilon$. This means that $\pi_{n}$ is $\epsilon$-independent of $\pi_{0},\dots, \pi_{n-1}$.

Without loss of generality, we can assume $\pi_i$ for $i \leq n-1$ is not $\epsilon$-near optimal (otherwise, we have already found a near optimal policy).  This implies that for the sequence $\{\pi_0,\dots, \pi_n\}$, we have that $\pi_i$ ($i\leq n$) is $\epsilon$-independent of all its predecessors. By definition of the distribution Eluder dimension, we have that $n \leq  d_{\epsilon} $. This implies that $\delta$ needs to be small enough such that:
\begin{align*}
\delta \leq  \frac{\epsilon^2}{ 4 d_{\epsilon}  }.
\end{align*}

Recall that our confidence interval is set as $\delta =  4\sqrt{\frac{ \ln(2 |\Pcal| N /\delta)  }{M}} + \frac{ 2\ln\left(2 |\Pcal| N / \delta \right)  }{M} \leq  4\sqrt{\frac{ \ln(2 |\Pcal| d_{\epsilon} /\delta)  }{M}} + \frac{ 2\ln\left(2 |\Pcal| d_{\epsilon} / \delta \right)  }{M}$. We can verify that by setting $M$ as:
\begin{align*}
M = \frac{256 d_{\epsilon}^2 \ln( 2|\Pcal| d_{\epsilon}/\delta)  }{\epsilon^4} + \frac{8 d_{\epsilon} \ln(2 |\Pcal| d_{\epsilon} /\delta )  }{\epsilon^2}, 
\end{align*} it is enough to ensure that $\delta \leq \epsilon^2 / (4 d_{\epsilon})$.
\end{proof}


==> eluder_generalization.tex <==
\section{Distributional Eluder Dimension}

\begin{algorithm}[t!]
	\begin{algorithmic}[1]	
		\REQUIRE  MDP $\mathcal{M}$, inputs $(M, \mathcal{P}, \Pi)$
		\STATE Initialize $\pi_0$
		\STATE Set policy-cover $\boldpi_0 = \{\pi_0\}$ 
        \FOR{$n = 0 \to N-1$}
        		\STATE Draw two datasets $\Dcal_1 = \{s_i,a_i,s_i'\}_{i=1}^M$ and $\Dcal_2 = \{s_i,a_i,s_i\}_{i=1}^M$, independently, where $s_i,a_i \sim d^{\boldpi_n}$, and $s'\sim P^\star(\cdot | s_i,a_i)$
        	       \STATE \emph{Fit model} (MLE) with data from policy-cover $\boldpi_{n}$            
	       \begin{align}
            \label{eq:mle}
            	\widehat{P}_n := \argmax_{P\in\mathcal{P}}\sum_{s,a,s'\in\Dcal_1} \ln P(s'|s,a)
		\end{align}
		%\STATE Draw another fresh $M$ data points, $\Dcal_n = \{s_i,a_i,s_i'\}$ with $si,$
		\STATE Set confidence region around the MLE $\widehat{P}_n$: $$\Pcal_n = \Big\{P\in\Pcal: \sum_{(s,a,s')\in\Dcal_2} \| \widehat{P}_{n;s,a} - P_{s,a}  \|^2_{1}  \leq \delta \Big\}$$
		%\STATE Set reward bonus $b_n$ as in Eq.~\ref{eq:reward_bonus}%Define bonus $b_n(s,a) := c \sqrt{\phi(s,a)^{\top} \widehat\Sigma_n^{-1}\phi(s,a)}$ 
		\STATE Plan: $\{\pi_{n+1}, \widetilde{P}_n \}= \argmax_{\pi\in\Pi, P\in\Pcal_n} V^{\pi}_{P}$ 
		%$\pi_{n+1} = \text{OP}\left( \Pi, r +  \widehat{b}_n, \widehat{P}_n,  \right)$            %\State Set absorbing MDP $\widetilde{\Mcal}_n$ based on $\widehat{\Sigma}_{n}$ and the MLE $\widehat{P}_n$ (Eq.~\ref{eq:absorbing_est})
            %\State \emph{Planning} in absorbing MDP: $\pi_{n+1} = \text{OP}\left(\widetilde{\Mcal}_n\right)$
            \STATE Update \emph{policy-cover}: $\boldpi_{n+1}  = \boldpi_n \oplus \{\pi_{n+1}\}$
            %\State Define $\rho_t := \left(\rho + (\sum_{i=0}^{n} d_n / (n+1))\right)/2$.
            %\State Collect data: $\{x_i, u_i, x'_{i}\}_{i=1}^K$ where $x_i,u_i \sim \rho_t$, $x'_i\sim P^\star_{x_i,u_i}$
            %\State Constrained Least Square: $\widehat{W}_n = \argmin_{W:\|W\|\leq M} \sum_{i=1}^K \| W\phi(x_i,u_i) - x'_{i} \|_2^2$.
            %\State Planning: $\pi_{n+1} = \argmin_{\pi\in\Pi} J(\pi; \widehat{W}_n)$
        \ENDFOR
         \end{algorithmic}
	\caption{{\small{Optimism-Driven \& Policy-cover guided MBRL}}}
\label{alg:dagger_1}
\end{algorithm}




In this section, we introduce the new structural complexity measure, \emph{Distributional Eluder Dimension}, for model-based RL. Previous definitions of Eluder dimension \cite{russo2014learning,osband2014model} concern about the worst case sequence of state action pairs, which works for one-step bandit problem, thus fails to take the property of the MDP and policy class into consideration. 

In contrast, our new distributional Eluder dimension definition takes both model class $\Pcal$ and policy class $\Pi$ as inputs, and considers quantities that are derived from the interaction of models, policies, and the underlying ground truth transition. The definition considers a sequence of policies rather than a sequence of state-action pairs. Given $\epsilon\in\mathbb{R}^+$,  and a sequence of policies $\pi_0,\dots, \pi_{t}$, let us define $w_{k}$ for $k\in [t]$ as follows. 
\begin{align*}
w_k = \sup_{(P,P')\in \widetilde{\Pcal}_k} \EE_{s,a\sim d^{\pi}}\left\| P(\cdot | s,a) - P'(\cdot | s,a)   \right\|_{1}, 
\end{align*}  where $\widetilde{\Pcal}_k$ is defined as:
{\scriptsize{\begin{align*}
\widetilde{\Pcal}_k = \left\{ (P, P'):  \sqrt{\sum_{i=0}^{k-1} \left(\EE_{s,a\sim d^{\pi_i}}\left\| P(\cdot | s,a) - P'(\cdot | s,a) \right\|_{tv}\right)^2}\leq \epsilon. \right\}.
\end{align*}
}}


Intuitively, $\widetilde{\Pcal}_k$ contains pairs of models that agree with each other on the policy cover $\pi_0,\dots, \pi_{k-1}$, while $w_k$ is the maximum possible disagreement between any two models from $\widetilde{P}_{k}$ when measured under the new distribution $d^{\pi_k}$. Small distributional eluder dimension means that we cannot find too many different state-action distributions. 
\begin{definition}[Distributional Eluder Dimension] The $\epsilon$ Distributional Eluder Dimension $d_{E}(\epsilon)$ is defined as the length of the longest sequence of $\pi_1,\pi_2,\dots, \pi_t$, such that for $w_k \geq \epsilon$ for all $k \leq t$.
 \end{definition}


\iffalse
we say that a policy $\pi$ is $\epsilon$-independent of $\pi_0,\dots, \pi_{t-1}$, if there exists $P\in\Pcal$ and $P'\in\Pcal$, such that
\begin{align*}
\EE_{s,a\sim d_h^{\pi}}\left\| P_h(\cdot | s,a) - P'_h(\cdot | s,a)   \right\|_{tv} \geq \epsilon, 
\end{align*} while $P$ and $P'$ agrees on previous policies, i.e., 
\begin{align*}
\sqrt{\sum_{i=0}^{t-1} \left(\EE_{s,a\sim d_h^{\pi_i}}\left\| P_h(\cdot | s,a) - P'_h(\cdot | s,a) \right\|_{tv}\right)^2}\leq \epsilon.
\end{align*}The $\epsilon$-independence intuitively means that $d^{\pi_t}_h$ is not that similar to all previous state-action distributions $d_h^{\pi_0},\dots d^{\pi_{t-1}}_h$, since we can find two models that agree with each other on $d_h^{\pi_0},\dots d^{\pi_{t-1}}_h$, but fails to agree on $d_h^{\pi_t}$.

Distributional Eluder dimension $d_{\epsilon}$ is the longest such sequence of policies $\{\pi_0,\dots, \pi_{d_{\epsilon}-1}\}$ such that for any $i \in [d]$, $\pi_i$ is $\epsilon$-independent of $\pi_0,\dots, \pi_{i-1}$.
\fi

Together with the new structural complexity measure, we also provide the algorithm (Algorithm~\ref{alg:dagger_1}), named \emph{Optimism-driven and Policy-cover guided MBRL},
 that achieves sample complexity scaling polynomially with respect to the distributional Eluder dimension. The algorithm works as follows. Given the policy cover $\{\pi_0,\dots, \pi_{n}\}$, we train an empirical model via MLE $\widehat{P}$ under the distribution induced by the uniform mixture $\boldpi_n$ of the cover:
%\begin{align*}
%\widehat{P}_{n;h} =  \max_{P\in\Pcal} \sum_{i=1}^{M} \ln\left( P(s_i' | s_i, a_i)  \right),
%\end{align*} where $s_i, a_i \sim d^{\boldpi_n}_h$,  and $s_i' \sim P^\star_h(\cdot | s_i,a_i)$. MLE ensures that:
%\begin{align*}
%\EE_{s,a\sim d^{\boldpi_n}_h} \left\| \widehat{P}_{n;h}(\cdot | s,a) - P^\star_h(\cdot| s,a)   \right\|^2_{1} \leq \frac{ 2\ln\left( |\Pcal| / \delta \right) }{M}.
%\end{align*} 
We then define a confidence region $\widetilde{P}_n$ centered at $\widehat{P}_n$ based on empirical samples from the mixture policy $\boldpi_n$. The confidence region size $\delta$ is set such that $\widetilde{P}_n$ contains $P^\star$ with high probability.  
%This defines confidence regions, i.e., for all $h\in [H]$, denote $\Pcal_{n;h}$ as the following ball centered at $\widehat{P}_{n;h}$:
%\begin{align*}
%\Pcal_{n;h} = \left\{ P\in \Pcal: \EE_{s,a\sim d^{\boldpi_n}_h} \left[ \Delta(\widehat{P}_{n;h}; s,a)^2\right] \leq \frac{ 2\ln\left( |\Pcal| / \delta \right) }{M}   \right\}.
%\end{align*}
To select $\pi_{n+1}$, we pick the most optimistic model via the following constrained optimization:
$(\pi_{n+1}, \widetilde{P}_n) = \argmax_{\pi\in\Pi, P\in\Pcal} V^{\pi}_{P}$. 

To link the algorithm to the distributional Eluder dimension, we note that $\widehat{P}_n$ indeed contains models $P$ (including the optimistic model $\widetilde{P}_n$) that agrees with $P^\star$ under the distribution of the policy cover $\boldpi_n$. On the other hand, if $\pi_{n+1}$ is not a near optimal policy, then we can claim that we find a new policy $\pi_{n+1}$ such that $\widetilde{P}_n$ does not agree with $P^\star$ under its distribution $d^{\pi_{n+1}}$. Bounded distributional Eluder dimension implies that we cannot find too many different state-action distributions, thus ensuring that the algorithm will find near optimal policies with bounded number of iterations.  The following theorem summarizes the sample complexity of Algorithm~\ref{alg:dagger_1}.

\begin{theorem}[Sample Complexity of Alg.~\ref{alg:dagger_1}] Set $\epsilon \in (0,H)$ and $\delta\in(0,1)$.  Denote $d := d_{E}(\epsilon)$. With $N = d$, and $M = \Theta\left(\frac{ d^2 \ln( 2|\Pcal| d_{\epsilon}/\delta)  }{\epsilon^4}\right)$, Alg.~\ref{alg:dagger_1} finds a policy $\pi\in \{\pi_0,\dots, \pi_{N-1}\}$, such that $V^{\pi} \geq V^\star - \epsilon$, with total number of samples $\widetilde{O}\left( \frac{ d^3 \ln( 2|\Pcal| d_{\epsilon}/\delta)  }{\epsilon^4}  \right)$.
\end{theorem}
Here in $\widetilde{O}$ we ignore log terms that only contains $d, \epsilon, H, \epsilon, \delta$. Note that $\ln(|\Pi|)$ is considered as the complexity of our function class $\Pcal$.

%& \text{s.t.,}  P_h \in \Pcal_{n;h}, \forall h\in [H],
%\end{align*} and $\pi_{n+1}$ is the optimal solution of the above constrained optimization program. 






==> macros.tex <==
%!TEX root = corruption_main.tex
\newcommand{\LR}{\mathrm{LR}}
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calZ}{\mathcal{Z}}
\newcommand{\pl}{(1)}
\newcommand{\kl}{_{k,\ell}}
\newcommand{\klh}{_{k,\ell;h}}
\newcommand{\klpr}{_{k,\ell'}}
\newcommand{\klprh}{_{k,\ell';h}}
\numberwithin{equation}{section}


\newcommand{\wkl}{\weight\kl}
\newcommand{\wklh}{\weight\klh}
\newcommand{\nbar}{\overline{n}}
\newcommand{\nbark}{\nbar_k}
\newcommand{\eventproblelst}{\mathcal{E}^{\mathrm{lead},\le\lst}}
\newcommand{\eventprobl}{\mathcal{E}^{\mathrm{lead},\ell}}

\newcommand{\eventvalconc}{\mathcal{E}^{\mathrm{val,conc}}}
\newcommand{\eventprobconc}{\mathcal{E}^{\mathrm{prb,conc}}}
\newcommand{\xaxpr}{(x,a,x')}
\newcommand{\goodeps}{\mathcal{K}_{\mathrm{good}}}
\newcommand{\advrange}{\adv^{\mathrm{range}}}
\newcommand{\corrupt}{\mathbf{C}}
\newcommand{\Err}{\mathrm{Err}}



\newcommand{\Klst}{\lst}
\newcommand{\jh}{_{j;h}}
\newcommand{\jhpl}{_{j;h+1}}
\newcommand{\eventsub}{\calE^{\mathrm{subsmp}}}
\newcommand{\klsthpl}{_{k,\lst;h+1}}
\newcommand{\hpl}{_{h+1}}
\newcommand{\klhpltwo}{_{k,l;h+2}}
\newcommand{\xpr}{x'}
\newcommand{\klihpl}{_{k,\ell,i;h+1}}
\newcommand{\lmaxj}{\lmax_j}
\newcommand{\alphali}{\alpha_{\ell,i}}
\newcommand{\iset}{\left\{\mathrm{sb},\mathrm{gl}\right\}}
\newcommand{\corruptk}{\corrupt_k}
\newcommand{\didcorruptk}{\didcorrupt_k}
\newcommand{\eventconc}{\mathcal{E}^{\mathrm{conc}}}
 \newcommand{\klihpr}{_{k,\ell,i;h'}}

\newcommand{\boundlead}{\bound^{\mathrm{lead}}}
\newcommand{\boundcross}{\bound^{\mathrm{cross}}}
\newcommand{\boundtotal}{\bound^{\mathrm{total}}}
\newcommand{\xau}{(x,a;u)}
\newcommand{\bound}{\mathbf{B}}
\newcommand{\delv}{\Delta \vup}

\newcommand{\Errlead}{\Err^{\mathrm{val}}}
\newcommand{\klglb}{_{k,\ell,\mathrm{gl}}}
\newcommand{\klsub}{_{k,\ell,\mathrm{sb}}}
\newcommand{\klelst}{_{k,\le \lst}}
		\newcommand{\klst}{_{k,\lst}}

	\newcommand{\Pikl}{\Pi_{k}^{\ell}}
	\newcommand{\Piklelst}{\Pi_{k}^{\le\lst}}
\newcommand{\Pik}{\Pi_k}
\newcommand{\kli}{_{k,l,i}}
\newcommand{\klpl}{_{k,\ell+1}}
\newcommand{\klminh}{_{k,\ell-1;h}}
\newcommand{\piucb}[1]{\boldpi^{\mathrm{ucb},#1}}
\newcommand{\boldlk}{\boldl_k}
\newcommand{\Finite}[1]{\left[#1\right]_{<\infty}}
\newcommand{\nk}{n_k}
\newcommand{\nkl}{n_{k,\ell}}
\newcommand{\robustLfactor}{\Lfactor^{\mathrm{rbst}}}
\newcommand{\klih}{_{k,\ell,i;h}}
\newcommand{\Index}{\mathcal{I}}
		\newcommand{\klhpl}{_{k,\ell,h+1}}
\newcommand{\lfin}{\boldl^{\mathrm{fin}}}
\newcommand{\lmax}{\boldl^{\mathrm{max}}}
\newcommand{\klsth}{_{k,\lst;h}}
	\newcommand{\lst}{\ell_{\star}}
\newcommand{\Regret}{\mathrm{Regret}}

\newcommand{\pigreedboldl}{\pi^{\mathrm{ucb},\,(\boldl)}}
	\newcommand{\pigreedboldlk}{\pi^{\mathrm{ucb},\,(\boldl)}_k}
	\newcommand{\pigreedboldlkk}{\pi^{\mathrm{ucb},\,(\boldl_k)}_k}
\newcommand{\distlayer}{\mu_{\mathrm{layer}}}
 
\newcommand{\boldpik}{\boldsymbol{\pi}_k}
\newcommand{\boldpil}{\boldsymbol{\pi}^{\ell}}
\newcommand{\boldpilk}{\boldsymbol{\pi}^{\ell}_k}

\newcommand{\boldpilel}{\boldsymbol{\pi}^{\le\ell}}
\newcommand{\boldpilelst}{\boldsymbol{\pi}^{\le\lst}}


\newcommand{\boldpilelk}{\boldsymbol{\pi}^{\le\ell}_k}
\newcommand{\boldpilelstk}{\boldsymbol{\pi}^{\le\lst}_k}
\newcommand{\ellset}{\mathscr{L}}
\newcommand{\ellsetl}{\ellset_{\ell}}
\newcommand{\xkhakh}{(\matx\kh,\mata\kh)}
\newcommand{\xjhajh}{(\matx\jh,\mata\jh)}

\newcommand{\klplh}{_{k,\ell+1;h}}
\newcommand{\oplustau}{\oplus_{\tau}}
\newcommand{\oplush}{\oplus_{h}}
\newcommand{\oplushbar}{\oplus_{\hbar}}
\newcommand{\vsthpl}{\vst_{h+1}}
\newcommand{\xah}{(x,a,h)}
\newcommand{\gap}{\mathrm{gap}}
\newcommand{\gapmin}{\gap_{\min}}
\newcommand{\clip}[2]{\operatorname{clip}\left[#2|#1\right]}
\newcommand{\clipmid}[2]{\operatorname{clip}\left[#2\mid\,#1\right]}

\newcommand{\cliptil}[2]{\widetilde{\operatorname{clip}}\left[#2|#1\right]}

\newcommand{\advlucbhalfclip}{\dot{\adv}^{\mathrm{lucb}}}
 \newcommand{\advhalfclip}{\dot{\adv}}
 \newcommand{\phatk}{\phat_k}
\newcommand{\rhatk}{\rhat_k}
 \newcommand{\advlucbfullclip}{\ddot{\adv}^{\mathrm{lucb}}}
 \newcommand{\advfullclip}{\ddot{\adv}}
\newcommand{\gaph}{\mathrm{gap}_h}
\newcommand{\epsclip}{\epsilon_\mathrm{clip}}
\newcommand{\vsth}{\vst_h}
\newcommand{\mup}{\overline{\calM}}
\newcommand{\mlow}{\underline{\calM}}
\newcommand{\mlowk}{\mlow_k}
\newcommand{\mupk}{\mup_k}
\newcommand{\vupk}{\vup_k}
\newcommand{\vlowk}{\vlow_k}
\newcommand{\qlowk}{\qlow_k}
\newcommand{\qupk}{\qup_k}
\newcommand{\pigreedk}{\pigreed_k}
\newcommand{\ofx}{(x)}
\newcommand{\ofxh}{(x_h)}
\newcommand{\pisth}{\pist_h}
\newcommand{\xhah}{(x_h,a_h)}


\renewcommand{\ast}{a^\star}
\newcommand{\xast}{(x,\ast)}
\newcommand{\qsth}{\qst_h}
\newcommand{\bolda}{\mathbf{a}}
\newcommand{\poly}{\mathrm{poly}}
\newcommand{\activeset}{\mathscr{A}}
\newcommand{\activesetk}{\activeset_k}
\newcommand{\tuple}{\mathscr{T}}
\newcommand{\tuplek}{\tuple_k}
\newcommand{\Kpl}{K^{\pl}}
\newcommand{\matz}{\mathbf{z}}
\newcommand{\matxpl}{\matx^{\pl}}
\newcommand{\matypl}{\maty^{\pl}}
\newcommand{\calEtil}{\widetilde{\mathcal{E}}}
\newcommand{\kclass}{\mathscr{K}}
\newcommand{\lossid}[1]{\mathcal{L}_{\mathrm{id},#1}}

\newcommand{\advlucb}{\adv^{\mathrm{lucb}}}
\newcommand{\advlowgreed}{\advlow^{\mathrm{lcb}}}


\newcommand{\boldl}{\boldsymbol{\ell}}


\newcommand{\valf}{\boldsymbol{V}}
\newcommand{\vst}{\valf^{\star}}
\newcommand{\qst}{\qf^{\star}}
\newcommand{\pist}{\pi^{\star}}


\newcommand{\qf}{\boldsymbol{Q}}
\newcommand{\vup}{\bar{\valf}}
\newcommand{\qup}{\bar{\qf}}
\newcommand{\qlow}{\makelow{\qf}}
\newcommand{\vlow}{\makelow{\valf}}

\newcommand{\qcirc}{\mathring{\qf}}
\newcommand{\vcirc}{\mathring{\valf}}
\newcommand{\pibar}{\overline{\pi}}
\newcommand{\adv}{\mathbf{A}}

\newcommand{\advcirc}{\mathring{\adv}}

\newcommand{\occ}{\boldsymbol{\omega}}

\newcommand{\phat}{\widehat{p}}
\newcommand{\rhat}{\widehat{r}}

\newcommand{\rhatkhl}{\rhat_{k,h,\ell}}
\newcommand{\khl}{_{k;h;l}}
\newcommand{\khbar}{_{k;\hbar}}

\newcommand{\khboldl}{_{k;h,\boldl}}

\newcommand{\khlpr}{_{k,h,l'}}
\newcommand{\khpl}{_{k;h+1}}
\newcommand{\khpr}{_{k;h'}}

\newcommand{\khlh}{_{k,h,\boldl_h}}
\newcommand{\xa}{(x,a)}


\newcommand{\makelow}[1]{\mkern2mu\underline{\mkern-2mu#1\mkern-4mu}\mkern4mu }


\newcommand{\bonus}{\boldsymbol{b}}
\newcommand{\bonuskhl}{\bonus_{k,h,\ell}}
\newcommand{\bonusbar}{\overline{\bonus}}
\newcommand{\bonuscirc}{\mathring{\bonus}}

\newcommand{\nkhl}{n_{k,h,\ell}}
\newcommand{\Lfactor}{\mathbf{L}}
\newcommand{\Lcorrupt}{\mathbf{L}_{\mathrm{crpt}}}

\newcommand{\cbon}{c_{\bonus}}
\renewcommand{\hbar}{\tau}
\newcommand{\hboldbar}{\overline{\boldsymbol{\tau}}}


\renewcommand{\ast}{a^\star}

\newcommand{\kh}{_{k;h}}
\newcommand{\boldpi}{\boldsymbol{\pi}}
\newcommand{\pigreed}{\pi^{\mathrm{ucb}}}
\newcommand{\piexp}{\pi^{\mathrm{exp}}}
\newcommand{\pimix}{\pi}
\newcommand{\pilcb}{\pi^{\mathrm{lcb}}}
\newcommand{\calMlow}{\makelow{\calM}}
\newcommand{\advlow}{\makelow{\adv}}
\newcommand{\bonuslow}{\makelow{\bonus}\,}


\newcommand{\weight}{\boldsymbol{\omega}}
\newcommand{\weighthbar}{\weight^{\hbar}}

\newcommand{\khhbar}{_{k,h;\hbar}}
\newcommand{\khhboldbar}{_{k,h;\hboldbar}}
\newcommand{\dens}{\rho}
\renewcommand{\colon}{{\,:\,}}
\newcommand{\calM}{\mathcal{M}}

\newcommand{\calMbar}{\overline{\calM}}
\newcommand{\pbar}{\overline{p}}
\newcommand{\rbar}{\overline{r}}

\newcommand{\states}{\mathcal{X}}
\newcommand{\actions}{\mathcal{A}}
\newcommand{\outputs}{\mathcal{Y}}
\newcommand{\matx}{\mathbf{x}}
\newcommand{\mata}{\mathbf{a}}

\newcommand{\Gclass}{\mathscr{G}}
\newcommand{\Ust}{U_{\star}}
%\newcommand{\Vst}{V_{\star}}
\newcommand{\sfP}{\mathsf{P}}

\newcommand{\Ast}{A_{\star}}
\newcommand{\Bst}{B_{\star}}
\newcommand{\Kst}{K_{\star}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\Khat}{\widehat{K}}
\newcommand{\matU}{\mathbf{U}}
\newcommand{\matDel}{\boldsymbol{\Delta}}
\newcommand{\Rhat}{\widehat{R}}

\newcommand{\Proj}{\mathrm{Proj}}
\newcommand{\ProjK}{\mathrm{Proj}_{\Kst}}
\newcommand{\ProjKzero}{\mathrm{Proj}_{\mathbf{0} \oplus \Kst}}
\newcommand{\veczero}{\mathbf{0}}

\newcommand{\Stief}{\mathrm{Stief}}
\newcommand{\nablabar}{\overline{\nabla}}
\newcommand{\nablacheck}{\check{\nabla}}
\newcommand{\fcheck}{\check{f}}
\newcommand{\Gcheck}{\check{G}}

\newcommand{\calK}{\mathcal{K}}
\newcommand{\calE}{\mathcal{E}}

\newcommand{\Rcheck}{\check{R}}

\newcommand{\xbar}{\overline{x}}
\newcommand{\xcheck}{\check{x}}


%comments

%ceiling
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

%theorems
{
 \theoremstyle{plain}
      \newtheorem{asm}{Assumption}
}
\newtheorem{nono-theorem}{Theorem}[]
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{claim}[theorem]{Claim}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{fact}[theorem]{Fact}
%\theoremstyle{remark}
%\newtheorem*{rem}{Remark}
\newtheorem*{note}{Note}

\newtheorem{prop}[theorem]{Proposition}
\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{example}{Example}[section]
\newtheorem{exc}{Exercise}[section]
\newtheorem{rem}{Remark}[section]
\newtheorem{obs}{Observation}[section]


%probability
\renewcommand{\Pr}{\mathbb{P}}
\newcommand{\Exp}{\mathbb{E}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\Cov}{\mathrm{Cov}}

\newcommand{\Law}{\mathrm{Law}}
\newcommand{\Leb}{\mathrm{Lebesgue}}

\newcommand{\unifsim}{\overset{\mathrm{unif}}{\sim}}
\newcommand{\iidsim}{\overset{\mathrm{i.i.d.}}{\sim}}
\newcommand{\probto}{\overset{\mathrm{prob}}{\to}}
\newcommand{\ltwoto}{\overset{L_2}{\to}}

\newcommand{\info}{\mathbf{i}}
\newcommand{\KL}{\mathrm{KL}}
\newcommand{\Ent}{\mathrm{Ent}}
\newcommand{\TV}{\mathrm{TV}}
\newcommand{\rmd}{\mathrm{d}}

%math operators
\newcommand{\median}{\mathrm{Median}}
\newcommand{\range}{\mathrm{range}}
\newcommand{\im}{\mathrm{im }}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\spec}{\mathrm{spec}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\Diag}{\mathrm{Diag}}
\newcommand{\sign}{\mathrm{sign\ }}
\newcommand{\abs}{\mathrm{abs\ }}

%norms
\newcommand{\op}{\mathrm{op}}
\newcommand{\F}{\mathrm{F}}
\newcommand{\dist}{\mathrm{dist}}

% logical
\renewcommand{\implies}{\text{ implies }}
\renewcommand{\iff}{\text{ iff }}
\newcommand{\matX}{\mathbf{X}}
\newcommand{\matbeta}{\boldsymbol{\beta}}
\newcommand{\mattheta}{\boldsymbol{\theta}}

\newcommand{\betast}{\matbeta^*}
\newcommand{\betahat}{\widehat{\matbeta}}

\newcommand{\thetast}{\mattheta^*}
\newcommand{\thetahat}{\widehat{\mattheta}}
\newcommand{\supp}{\mathrm{supp}}


\newcommand{\matw}{\mathbf{w}}
\newcommand{\maty}{\mathbf{y}}


%Number Spaces
\renewcommand{\Im}{\mathfrak{Im }}
\renewcommand{\Re}{\mathfrak{Re }}
\newcommand{\N}{\mathbb{Z}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\I}{\mathbb{I}}
\newcommand{\Q}{\mathbb{Q}}

%Vector Spaces
\newcommand{\PD}{\mathbb{S}_{++}^d}
\newcommand{\sphered}{\mathcal{S}^{d-1}}




% Asymptotics
\DeclareMathOperator{\BigOm}{\mathcal{O}}
\newcommand{\BigOh}[1]{\BigOm\left({#1}\right)}
\DeclareMathOperator{\BigOmtil}{\widetilde{\mathcal{O}}}
\newcommand{\BigOhTil}[1]{\BigOmtil\left({#1}\right)}
\DeclareMathOperator{\BigTm}{\Theta}
\newcommand{\BigTheta}[1]{\BigTm\left({#1}\right)}
\DeclareMathOperator{\BigWm}{\Omega}
\newcommand{\BigThetaTil}[1]{\widetilde{\BigTm}\left({#1}\right)}
\newcommand{\BigOmega}[1]{\BigWm\left({#1}\right)}
\DeclareMathOperator{\LittleOm}{\mathrm{o}}
\newcommand{\LittleOh}[1]{\LittleOm\left({#1}\right)}
\DeclareMathOperator{\LittleWm}{\omega}
\newcommand{\LittleOmega}[1]{\LittleWm\left({#1}\right)}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\logdet}{log\,det}

\newcommand{\Rsimple}{\mathcal{R}_{\mathrm{simp}}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\actst}{a_*}
\newcommand{\acthat}{\widehat{a}}


\newcommand{\lasso}{\mathsf{lasso}}
\newcommand{\four}{\mathscr{F}}
\newcommand{\LS}{\mathsf{LS}}
\newcommand{\Alg}{\mathsf{Alg}}


\newcommand{\vi}{\matv^{(i)}}

% Complexity Classes
\newcommand{\SAT}{\mathit{SAT}}
\renewcommand{\P}{\mathbf{P}}
\newcommand{\NP}{\mathbf{NP}}
\newcommand{\coNP}{\co{NP}}
\newcommand{\co}[1]{\mathbf{co#1}}

%%%%%%PG%%%%%%%
\newcommand{\dboldpi}{d_{\boldpi}}
\newcommand{\dpi}{d_{\pi}}
\newcommand{\sink}{s^{\dagger}}
\newcommand{\abmdp}{\calM^{\dagger}}


%%%%% Akshay's macros %%%%%
\newcommand{\epsstat}{\varepsilon_{\textrm{stat}}}
\newcommand{\bellman}{\mathcal{T}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\qhat}{\widehat{Q}}
\newcommand{\vhat}{\widehat{V}}
\newcommand{\aphi}{A\circ\phi}
\newcommand{\supi}{^{(i)}}
\newcommand{\calV}{\mathcal{V}}
%\newcommand{\xhah}{(x_h,a_h)}
